DASA: Difficulty-Aware Semantic Augmentation for Speaker Verification

Data augmentation is vital to the generalization ability and robustness of deep neural networks (DNNs) models. Existing augmentation methods for speaker verification manipulate the raw signal, which are time-consuming and the augmented samples lack diversity. In this paper, we present a novel difficulty-aware semantic augmentation (DASA) approach for speaker verification, which can generate diversified training samples in speaker embedding space with negligible extra computing cost. Firstly, we augment training samples by perturbing speaker embeddings along semantic directions, which are obtained from speaker-wise covariance matrices. Secondly, accurate covariance matrices are estimated from robust speaker embeddings during training, so we introduce difficultyaware additive margin softmax (DAAM-Softmax) to obtain optimal speaker embeddings. Finally, we assume the number of augmented samples goes to infinity and derive a closed-form upper bound of the expected loss with DASA, which achieves compatibility and efficiency. Extensive experiments demonstrate the proposed approach can achieve a remarkable performance improvement. The best result achieves a 14.6% relative reduction in EER metric on CN-Celeb evaluation set.

==> 01_introduction_backup_v1.tex <==
\section{introduction}
\label{sec:introduction}

% 说话人验证是比较两个语音样本/话语，并判断它们是否由相同的说话人所说。
Speaker verification is to compare two speech utterances and verify whether they are spoken by the same speaker \cite{7298570}.
%It plays an important role in our daily life, such as biometric identification or smart-phone control.
% 由于语音识别技术在深度学习的推动下获得了巨大进展,说话人识别技术深受影响,越来越多的研究者们从传统的基于概率统计方法转移到基于深度学习方法。
%As speech recognition technology has made significant progress driven by deep neural networks, speaker recognition technology is deeply affected. More and more researchers have shifted from traditional probability-based methods \cite{4156202,dehak2010front} to DNN-based methods \cite{6854363,snyder2018x}.
% JFA \cite{4156202}
% i-vector \cite{dehak2010front}
% d-vector \cite{6854363}
% x-vector \cite{snyder2018x}
% ecapa \cite{desplanques2020ecapa}
% resnet \cite{he2016deep}
% 数据集对训练一个好的深度模型来说是至关重要的条件之一，因此音频数据的需求也与日俱增。
In recent years, deep neural networks (DNNs) have significant boosted advancements in speaker verification \cite{snyder2018x,he2016deep,desplanques2020ecapa} and even deliver the equal error rate (EER) less than 1\% in VoxCeleb1-O benchmark. Now speaker verification becomes a well-developed technology in our daily life, such as biometric identification or smart-phone control.

Despite the great success, current speaker verification systems are are far from satisfactory in real industrial scenarios, such as video analysis where the variations on ambient, channel and emotion could be arbitrary.
% 有点奇怪
% such as video analysis with arbitrary(non-standard?) ambient sound, channel number and speech emotion.

To obtain a robust performance in complex industrial scenarios, data augmentation is an essential technique which efficiently increases the diversity and quantity of training samples.
%
%The remarkable improvement in speaker verification technologies is not only attributed to the power of DNNs, but also the large scale datasets with annotated labels. 
%
%Datasets are one of the most critical conditions for training deep models, so the demand for audio data is also growing \cite{7298570}.
%
% 数据增强是提高模型泛化能力和鲁棒性的重要方法，它可以增加训练样本的数量和分布多样性，提高识别准确率。
%Data augmentation has been extensively studied for audio and speech recognition tasks. 
%It is an essential technique 
% for improving the robustness and generalization ability of models, 
%which can increase the quantity and diversity of existing training samples and improve recognition accuracy \cite{fujii2022data,yamamoto2019speaker}.
% 说话人验证中常用的数据增强方法包括加噪声、加混响和速度扰动。
%Data augmentation commonly used in speaker verification contains additive noises, reverberation and speed perturbation \cite{snyder2018x,ko2015audio}.
% The additive noise \cite{snyder2018x} randomly selects audio from the MUSAN \cite{snyder2015musan} dataset which consists of noises, music and speech to augment the original audio.
% Reverberation \cite{snyder2018x,https://doi.org/10.48550/arxiv.2206.11699} refers to convolving room impulse responses(RIR) with audio. The training signal is artificially reverberated by convolution with simulated RIRs.
% Speed perturbation is to randomly speed up or down each utterance with ratio 0.9 or 1.1, considering the utterances with different speeds from new speakers \cite{yamamoto2019speaker,ko2015audio}.
% 
% 这些conventional的数据增强方法，都是直接处理原始信号的音频级语音增强方法。使用这些techniques增强样本的多样性都有限，同时还会很大程度地减慢训练速度。
However, existing data augmentation techniques for speaker verification, e.g., additive noises, reverberation and speed perturbation, are raw signal level data augmentation,
which directly process the raw audio \cite{ko2015audio}.
The diversity of augmented samples with these methods is inherently limited.
Besides, these conventional methods will also introduce huge computing cost and I/O time for augmentation, which significantly slow down the model training.

% 幸运的是，一种提出的隐式语义数据增强方法（引用isda）执行保持类别身份信息的语义转换（引用MetaSAug），从语音特征空间的角度出发，巧妙地利用深度神经网络长于学习线性化表征的性质，按照特征均值和协方差矩阵组成的高斯分布进行采样得到的语义转换方向，可以生成许多新的实例（引用image by reason）。
% 同时，它无需训练任何辅助生成模型（如GAN等），并没有显式地进行实例增强过程，而是直接近似优化无穷扩增样本期望交叉熵损失的一个上界，最终可以在softmax函数的基础上将算法归化为一个全新的损失函数，几乎不引入任何额外计算或时间开销。
%Fortunately, a proposed implicit semantic data augmentation (ISDA) algorithm \cite{wang2019implicit,9332260} performs meaningful semantic transformation that preserves category identity information \cite{li2021metasaug}. 
%Inspired by this, we introduce ISDA into speaker verification for the first time. 

In this paper, inspired by implicit semantic data
augmentation (ISDA)\cite{wang2019implicit,9332260},
we propose a novel difficulty-aware semantic augmentation (DASA) approach to augment the training data in deep speaker embedding level rather than raw signal level.
Instead of augment the speech by processing the raw signal, the DASA performs meaningful semantic perturbation during speaker embedding learning. 

Firstly, during training, we estimates
covariance matrices of each speaker’s embedding, and then generates diversified samples by perturbing speaker embedding along semantic directions from a zero-mean normal distribution.

From the perspective of speaker embedding space, DASA cleverly takes advantage of the deep neural network's ability to learn linearized representations. The semantic transformation directions obtained by sampling a zero-mean normal distribution 
with dynamically estimated speaker-wise covariance matrices can generate many new augmented instances.


In addition, DASA does not train any auxiliary generative adversarial network (GAN) or explicitly perform the sample augmentation process. 
% to improve efficiency. 
Instead, it optimizes an upper bound of the expected cross-entropy (CE) loss of infinitely augmented samples. Finally, it can reduce the algorithm to a simple loss function with negligible additional computation and time cost.


%ISDA中准确估算协方差矩阵需要学到较好的embeddings。除模型结构外，损失函数在说话人特征中也起着关键作用。 使用损失函数学习到好的说话人特征的目标在于减少类内方差，增大类间的差距。最开始使用最多的softmax损失函数擅长将不同类别的说话人特征优化得更加分散,但是并不能很好地使相同类别的说话人特征变得更加紧凑（引用am-softmax那篇文章）。因此很多新的损失函数被提出来完成类内聚集且类间分散的目标。一些度量学习任务通过学习说话人特征的度量空间来进行说话人分类，但这种方法通常需要大量两元组、三元组或者组间样本(引用相关的几篇文章)，较难设计导致数据的分布并不一定均匀，训练结果的影响偏局部(引用real amsoftmax)，在模型训练过程收敛慢。
In ISDA, the estimation of exact covariance matrices requires good embeddings. However, the original ISDA \cite{wang2019implicit} is based on softmax training, which can not get discriminative embeddings in speaker verification. 
% which has poor performance in speaker verification. 
% Learning good speaker embeddings aims to reduce the intra-class variation and increase the inter-class difference. 
This is because the softmax loss only separates the embeddings from the different speakers, but it is not very good at optimizing the embeddings of the same speakers to be more compact.
To get optimal embeddings, many new loss functions are proposed \cite{7472652,li2017deep,wan2018generalized,8331118,liu2017sphereface,deng2019arcface}.
% to reduce the intra-class variation and increase the inter-class difference \cite{8331118,9023039}. 
% Some metric learning tasks perform speaker classification by learning the metric space of speaker features \cite{7472652,li2017deep,wan2018generalized}. However, these methods usually require many paired samples which are difficult to mine with
% % and lead to uniform data distribution  with
% ineffective and slow training\cite{li2022real}.
% % processes
% 随后提出了一些max-margin训练方法(引用)，其中表现较好的方法有am-softmax（引用）。通过把角度margin引入softmax中，直接作用在所有训练样本上，这些方法更关注类内的紧凑性，形式简单且可以将目标类和非目标类更好地分开。但是在训练过程中，每个样本的特征向量和真实说话人类别中心的角度基本都不相同。因此我们提出了一个与样本余弦角度呈负相关的难度系数，直接乘在原本的固定margin上，当训练样本和类中心的角度越大时，表明这个样本越困难，相乘后的margin值越大，对于较简单的训练样本，设置稍小的margin值就可以很好地区分开（引用dy）。基于难度感知的AM-softmax会更加关注那些通常导致较差结果的困难实例（引用da），进而学习到更均衡、更好的特征表示。
% Then there are several max-margin softmax losses\cite{8331118,liu2017sphereface,deng2019arcface}, 
among which additive-margin softmax (AM-Softmax) \cite{8331118} loss pays more attention to the intra-class compactness by introducing the angular margin into the softmax. 
% So it can explicitly reduce the intra-class variation and increase the inter-class difference.
% So it can get better embeddings for estimating covariance matrices. 
% Several max-margin softmax techniques \cite{8331118,liu2017sphereface,deng2019arcface} were subsequently proposed, among which additive-margin softmax (AM-Softmax) \cite{8331118} loss has better performance. 

% Therefore, this paper rationally deduces ISDA on AM-Softmax.

% suboptimal robust
But AM-Softmax sets a fixed angular margin for all samples, the angle between the embedding vector and the center of the speaker category is different for each sample. 
We are motivated by \cite{https://doi.org/10.48550/arxiv.2104.06094} and introduce difficulty-aware AM-Softmax (DAAM-Softmax) whose margin is negatively correlated with the cosine angle. 
% for the fixed initial margin. 
When the angle between the training sample and the class center is larger, the sample is more difficult, and the margin is higher \cite{zhou2020dynamic}. 
% For simple training utterances, setting a slightly smaller margin can distinguish well. 
DAAM-Softmax can alleviate over-optimization of easy samples, and can also solve under-optimization of difficult samples\cite{https://doi.org/10.48550/arxiv.2104.06094}. 
It will also learn optimal embeddings for estimating covariance matrices.

% 本文我们提出一种基于am-loss能感知难度的隐式语义数据增强方法
Finally, we innovatively derive a closed-form upper bound of the expected loss based on DAAM-Softmax. 
% and apply it to the speaker verification task. 
% The difficulty-aware AM-Softmax loss can adaptively add different margins according to instance difficulty.
% and help networks learn better features. 
% Different from traditional augmentation, ISDA does not need to process the raw speech signal and can efficiently achieve meaningful semantic transformations.
% in the deep feature space. 
%
%\begin{itemize}[itemsep=0pt,topsep=0pt,parsep=0pt,leftmargin=10pt]
%\item We rationally derive ISDA based on AM-Softmax and first apply it to speaker verification task, which implements semantic data augmentation in the speech embedding space with little extra cost.
%\item We introduce difficulty-aware margin loss to extract better features, which is applied to ISDA to estimate more accurate covariance matrices.
%\item The proposed method can combine with traditional data augmentation and is compatible with any model to achieve higher performance.
%\end{itemize}
%
%
%
In summary, our contributions are as follows:

\begin{itemize}[itemsep=0pt,topsep=0pt,parsep=0pt,leftmargin=10pt]
\item \textbf{Low computing cost}: Instead of augmenting the speech by processing the raw signal, DASA perform meaningful semantic perturbation in speaker embedding space with little extra computing cost.
\item \textbf{Good compatibility}: The proposed DASA approach can combine with traditional data augmentation and is compatible with any model to achieve better recognition performance.
\item \textbf{Outstanding improvement}: Extensive experiments 
conducted on VoxCeleb and CN-Celeb demonstrate the proposed method can obtain remarkable performance improvement.
\end{itemize}

==> 01_introduction_backup_v2.tex <==
\section{introduction}
\label{sec:introduction}

Speaker verification is to compare two speech utterances and verify whether they are spoken by the same speaker \cite{7298570}.
In recent years, deep neural networks (DNNs) have significant boosted advancements in speaker verification \cite{snyder2018x,he2016deep,desplanques2020ecapa}.  
% and even deliver the equal error rate (EER) less than 1\% in VoxCeleb1-O benchmark. 
Now speaker verification becomes an important technology in our daily life, such as biometric identification or smart-phone control. However, current speaker verification systems are still unsatisfactory in real industrial scenarios, 
% such as video analysis where the variations on ambient, channel and emotion could be arbitrary. 
%有点奇怪
such as video analysis with non-standard ambient sound, channel number and speech emotion.
Data insufficiency is one of the most critical challenges to robustness of performance in complex scenarios.

To address the problem of lacking data, data augmentation is an essential technique which efficiently increases the diversity and quantity of training samples.
However, existing data augmentation techniques for speaker verification, e.g., additive noises, reverberation and speed perturbation, are raw signal level data augmentation.
The diversity of augmented samples generated by these methods is inherently limited by the direct manipulation of the raw audio \cite{ko2015audio}.
Besides, these conventional methods will also introduce huge computing cost and I/O time for augmentation, which significantly slow down the model training speed.

Recently, in order obtain a more robust speaker verification system, many novel training strategies and augmentation schemes have been proposed.
For instance, 
\cite{yang2018generative,wu2019data} firstly use deep generative models, e.g, Generative Adversarial Networks (GANs), Variational Autoencoder (VAE), to learn the distribution of noisy speaker embeddings and generate sample new embeddings from the generative models learned distribution.
\cite{wang2020investigation} investigates the usage of SpecAugment\cite{park19e_interspeech} for speaker verification, which augment the data by masking the spectrogram during training. 
\cite{9362090} sample noise from the pure noise distribution and directly add it to clean embeddings to generate augmented embeddings.


However, above augmentation methods contain two weaknesses.
Firstly, computation and time costs are increasing. These methods may need to use complex deep generative models to explicitly augment samples, which will also slow down the training process of recognition models. 
Secondly, the compatibility of above augmentation methods are not good. %Some techniques change the model structure or rely on extra noise data, so data augmentation can not be performed directly on the original model and data.
%%最后一句话在表达什么？
Some techniques are derived and specialized on certain datasets, performing sub-optimally on different datasets.

%%第4段和第二段重复了，到底是哪些方法有缺点？前面引入的篇幅有点长
Fortunately, these problems can potentially be solved by the implicit semantic data augmentation (ISDA) approach \cite{wang2019implicit,9332260}.
%It does not require noise data or any auxiliary model, and does not change the model structure, so there is almost no extra computation and time cost. 
Noise data, auxiliary model and model modification are no longer required, and therefore, it eliminates extra computation and time cost.
ISDA first estimates speaker-wise covariance matrices according to speaker embeddings. Then it augments training data by translating speaker embeddings towards meaningful semantic directions sampled from a zero-mean normal distribution with the dynamically estimated covariance matrices \cite{li2021metasaug}. 
However, ISDA performs poorly in speaker verification tasks, because it is based on softmax training, unable to acquire the optimal embedding to estimate the appropriate covariance matrices. 

In this paper, we propose a novel difficulty-aware semantic augmentation (DASA) approach to augment the training data in deep speaker embedding level rather than raw signal level, from the point that more accurate covariance matrices requires optimal embeddings. Without changing the model structure, loss function plays a crucial role in speaker embeddings. 
We first use additive-margin softmax (AM-Softmax) \cite{8331118} to reduce the intra-class variation and increase the inter-class difference \cite{8331118,9023039}. 
After that, in order to solve over-optimization of easy samples and under-optimization of difficult samples, we are inspired by \cite{https://doi.org/10.48550/arxiv.2104.06094} and introduce difficulty-aware AM-Softmax (DAAM-Softmax) which can pay more attention to difficult samples. 
% to make the margin value positively correlated with the sample difficulty. 
Based on DAAM-Softmax, we can get the optimal embeddings for covariance matrices. 
Finally, We assume infinite augmentation and derive an upper bound of expected loss with DASA, which greatly saves computation and time cost.
% and pay more attention to difficult examples
% Instead of augment the speech by processing the raw signal, the DASA performs meaningful semantic perturbation during speaker embedding learning. 
In summary, our contributions are as follows:

\begin{itemize}[itemsep=0pt,topsep=0pt,parsep=0pt,leftmargin=10pt]
\item \textbf{Low computing cost}: Instead of augmenting the speech by processing the raw signal, DASA perform meaningful semantic perturbation in speaker embedding space with little extra computing cost.
\item \textbf{Good compatibility}: The proposed DASA approach can combine with traditional data augmentation and is compatible with any model to achieve better recognition performance.
\item \textbf{Outstanding improvement}: Extensive experiments 
conducted on VoxCeleb and CN-Celeb demonstrate the proposed method can obtain remarkable performance improvement.
\end{itemize}
